Time-dependent $CP$ violation results at Belle II

We report updates on time-dependent $CP$-violation observables at Belle II. The benchmark measurements of the $B^0$ lifetime $\tau_{B^0}$ and mixing frequency $\Delta m_d$ using flavor specific hadronic decays and the determination of the $CP$-violating phase $\sin2\phi_1$ in $b\to c\overline{c}s$ transitions have been performed using data collected between 2019-2021. These analyses use only half of the current available dataset and are still statistically limited, showing the excellent performance of the detector and readiness of the analysis tools. We present three new results on the effective value of $\sin2\phi_1$ in $b\to q\overline{q}s$ transitions, which are highly sensitive to generic non-Standard Model (SM) physics amplitudes, using the full dataset collected between 2019-2022.

==> belle2-symbols.tex <==
% Standard Belle II aliases
% A. Di Canto (16-Sep-2022)
% Based on:
%  - babarsym.tex (by D. Hitlin, D. MacFarlane, P. Dauncey, R. Waldi)
%  - lhcb-symbols-def.tex (by U. Egede, T. Skwarnicki, C. Parkes, R. Oldeman, P. Koppenburg)

\RequirePackage{xspace}
\RequirePackage{relsize}

%%%%%%%%%%%%%
% Experiments
%%%%%%%%%%%%%
\def\belletwo{\mbox{Belle~II}\xspace}
\def\belle  {\mbox{Belle}\xspace}
\def\lhcb {\mbox{LHCb}\xspace}
%\def\babar  {\mbox{BaBar}\xspace}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}\xspace}

%%%%%%%%%%%%%
% Particles
%%%%%%%%%%%%%
\def\Palpha      {\ensuremath{\alpha}\xspace}
\def\Pbeta       {\ensuremath{\beta}\xspace}
\def\Pgamma      {\ensuremath{\gamma}\xspace}                 
\def\Pdelta      {\ensuremath{\delta}\xspace}                 
\def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
\def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
\def\Pzeta       {\ensuremath{\zeta}\xspace}                 
\def\Peta        {\ensuremath{\eta}\xspace}                 
\def\Ptheta      {\ensuremath{\theta}\xspace}                 
\def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
\def\Piota       {\ensuremath{\iota}\xspace}                 
\def\Pkappa      {\ensuremath{\kappa}\xspace}                 
\def\Plambda     {\ensuremath{\lambda}\xspace}                 
\def\Pmu         {\ensuremath{\mu}\xspace}                 
\def\Pnu         {\ensuremath{\nu}\xspace}                 
\def\Pxi         {\ensuremath{\xi}\xspace}                 
\def\Ppi         {\ensuremath{\pi}\xspace}                 
\def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
\def\Prho        {\ensuremath{\rho}\xspace}                 
\def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
\def\Ptau        {\ensuremath{\tau}\xspace}                 
\def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
\def\Pphi        {\ensuremath{\phi}\xspace}                 
\def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
\def\Pchi        {\ensuremath{\chi}\xspace}                 
\def\Ppsi        {\ensuremath{\psi}\xspace}                 
\def\Pomega      {\ensuremath{\omega}\xspace}                 
\mathchardef\PDelta="7101
\mathchardef\PXi="7104
\mathchardef\PLambda="7103
\mathchardef\PSigma="7106
\mathchardef\POmega="710A
\mathchardef\PUpsilon="7107
\def\PA      {\ensuremath{A}\xspace}                 
\def\PB      {\ensuremath{B}\xspace}                 
\def\PC      {\ensuremath{C}\xspace}                 
\def\PD      {\ensuremath{D}\xspace}                 
\def\PE      {\ensuremath{E}\xspace}                 
\def\PF      {\ensuremath{F}\xspace}                 
\def\PG      {\ensuremath{G}\xspace}                 
\def\PH      {\ensuremath{H}\xspace}                 
\def\PI      {\ensuremath{I}\xspace}                 
\def\PJ      {\ensuremath{J}\xspace}                 
\def\PK      {\ensuremath{K}\xspace}                 
\def\PL      {\ensuremath{L}\xspace}                 
\def\PM      {\ensuremath{M}\xspace}                 
\def\PN      {\ensuremath{N}\xspace}                 
\def\PO      {\ensuremath{O}\xspace}                 
\def\PP      {\ensuremath{P}\xspace}                 
\def\PQ      {\ensuremath{Q}\xspace}                 
\def\PR      {\ensuremath{R}\xspace}                 
\def\PS      {\ensuremath{S}\xspace}                 
\def\PT      {\ensuremath{T}\xspace}                 
\def\PU      {\ensuremath{U}\xspace}                 
\def\PV      {\ensuremath{V}\xspace}                 
\def\PW      {\ensuremath{W}\xspace}                 
\def\PX      {\ensuremath{X}\xspace}                 
\def\PY      {\ensuremath{Y}\xspace}                 
\def\PZ      {\ensuremath{Z}\xspace}                 
\def\Pa      {\ensuremath{a}\xspace}                 
\def\Pb      {\ensuremath{b}\xspace}                 
\def\Pc      {\ensuremath{c}\xspace}                 
\def\Pd      {\ensuremath{d}\xspace}                 
\def\Pe      {\ensuremath{e}\xspace}                 
\def\Pf      {\ensuremath{f}\xspace}                 
\def\Pg      {\ensuremath{g}\xspace}                 
\def\Ph      {\ensuremath{h}\xspace}                 
\def\Pi      {\ensuremath{i}\xspace}                 
\def\Pj      {\ensuremath{j}\xspace}                 
\def\Pk      {\ensuremath{k}\xspace}                 
\def\Pl      {\ensuremath{l}\xspace}                 
\def\Pm      {\ensuremath{m}\xspace}                 
\def\Pn      {\ensuremath{n}\xspace}                 
\def\Po      {\ensuremath{o}\xspace}                 
\def\Pp      {\ensuremath{p}\xspace}                 
\def\Pq      {\ensuremath{q}\xspace}                 
\def\Pr      {\ensuremath{r}\xspace}                 
\def\Ps      {\ensuremath{s}\xspace}                 
\def\Pt      {\ensuremath{t}\xspace}                 
\def\Pu      {\ensuremath{u}\xspace}                 
\def\Pv      {\ensuremath{v}\xspace}                 
\def\Pw      {\ensuremath{w}\xspace}                 
\def\Px      {\ensuremath{x}\xspace}                 
\def\Py      {\ensuremath{y}\xspace}                 
\def\Pz      {\ensuremath{z}\xspace}                 

%% generic

\def\hpm  {\ensuremath{\Ph^\pm}\xspace} 
\def\hp     {\ensuremath{\Ph^+}\xspace} 
\def\hm    {\ensuremath{\Ph^-}\xspace}
\def\ellpm{\ensuremath{\ell^\pm}\xspace}
\def\ellp   {\ensuremath{\ell^+}\xspace}
\def\ellm  {\ensuremath{\ell^-}\xspace}

%% Leptons

\let\emi\en
\def\electron   {\ensuremath{\Pe}\xspace}
\def\en         {\ensuremath{\Pe^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{\Pe^+}\xspace}
\def\epm        {\ensuremath{\Pe^\pm}\xspace} 
\def\epem       {\ensuremath{\Pe^+\Pe^-}\xspace}
\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\mmu        {\ensuremath{\Pmu}\xspace}
\def\mup        {\ensuremath{\Pmu^+}\xspace}
\def\mun        {\ensuremath{\Pmu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\Pmu^+\Pmu^-}\xspace}
\def\mtau       {\ensuremath{\Ptau}\xspace}

\def\taup       {\ensuremath{\Ptau^+}\xspace}
\def\taum       {\ensuremath{\Ptau^-}\xspace}
\def\tautau     {\ensuremath{\Ptau^+\Ptau^-}\xspace}

\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {\ensuremath{\Pnu}\xspace}
\def\neub       {\ensuremath{\overline{\Pnu}}\xspace}
\def\nuenueb    {\ensuremath{\neu\neub}\xspace}
\def\neue       {\ensuremath{\neu_e}\xspace}
\def\neueb      {\ensuremath{\neub_e}\xspace}
\def\neueneueb  {\ensuremath{\neue\neueb}\xspace}
\def\neum       {\ensuremath{\neu_\mu}\xspace}
\def\neumb      {\ensuremath{\neub_\mu}\xspace}
\def\neumneumb  {\ensuremath{\neum\neumb}\xspace}
\def\neut       {\ensuremath{\neu_\tau}\xspace}
\def\neutb      {\ensuremath{\neub_\tau}\xspace}
\def\neutneutb  {\ensuremath{\neut\neutb}\xspace}
\def\neul       {\ensuremath{\neu_\ell}\xspace}
\def\neulb      {\ensuremath{\neub_\ell}\xspace}
\def\neulneulb  {\ensuremath{\neul\neulb}\xspace}

%% Gauge bosons and scalars

\def\g      {\ensuremath{\Pgamma}\xspace}
\def\H      {\ensuremath{\PH^0}\xspace}
\def\Hp     {\ensuremath{\PH^+}\xspace}
\def\Hm     {\ensuremath{\PH^-}\xspace}
\def\Hpm    {\ensuremath{\PH^\pm}\xspace}
\def\W      {\ensuremath{\PW}\xspace}
\def\Wp     {\ensuremath{\PW^+}\xspace}
\def\Wm     {\ensuremath{\PW^-}\xspace}
\def\Wpm    {\ensuremath{\PW^\pm}\xspace}
\def\Z      {\ensuremath{\PZ^0}\xspace}

%% Quarks

\def\quark     {\ensuremath{\Pq}\xspace}
\def\quarkbar  {\ensuremath{\overline \quark}\xspace}
\def\qqbar     {\ensuremath{\quark\quarkbar}\xspace}
\def\uquark    {\ensuremath{\Pu}\xspace}
\def\uquarkbar {\ensuremath{\overline \uquark}\xspace}
\def\uubar     {\ensuremath{\uquark\uquarkbar}\xspace}
\def\dquark    {\ensuremath{\Pd}\xspace}
\def\dquarkbar {\ensuremath{\overline \dquark}\xspace}
\def\ddbar     {\ensuremath{\dquark\dquarkbar}\xspace}
\def\squark    {\ensuremath{\Ps}\xspace}
\def\squarkbar {\ensuremath{\overline \squark}\xspace}
\def\ssbar     {\ensuremath{\squark\squarkbar}\xspace}
\def\cquark    {\ensuremath{\Pc}\xspace}
\def\cquarkbar {\ensuremath{\overline \cquark}\xspace}
\def\ccbar     {\ensuremath{\cquark\cquarkbar}\xspace}
\def\bquark    {\ensuremath{\Pb}\xspace}
\def\bquarkbar {\ensuremath{\overline \bquark}\xspace}
\def\bbbar     {\ensuremath{\bquark\bquarkbar}\xspace}
\def\tquark    {\ensuremath{\Pt}\xspace}
\def\tquarkbar {\ensuremath{\overline \tquark}\xspace}
\def\ttbar     {\ensuremath{\tquark\tquarkbar}\xspace}

%% Light mesons

\def\pion  {\ensuremath{\Ppi}\xspace}
\def\piz   {\ensuremath{\pion^0}\xspace}
\def\pizs  {\ensuremath{\pion^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pion^0\pion^0}\xspace}
\def\pip   {\ensuremath{\pion^+}\xspace}
\def\pim   {\ensuremath{\pion^-}\xspace}
\def\pipi  {\ensuremath{\pion^+\pion^-}\xspace}
\def\pipm  {\ensuremath{\pion^\pm}\xspace}
\def\pimp  {\ensuremath{\pion^\mp}\xspace}
\def\pisoft{\ensuremath{\pion_s}\xspace}
\def\kaon  {\ensuremath{\PK}\xspace}
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em \PK}{}\xspace}% do NOT use ensuremath here
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{\kaon^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{\kaon^+}\xspace}
\def\Km    {\ensuremath{\kaon^-}\xspace}
\def\Kpm   {\ensuremath{\kaon^\pm}\xspace}
\def\Kmp   {\ensuremath{\kaon^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
% \def\KS    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle S}}\xspace} 
% \def\KL    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle L}}\xspace} 
\def\KS    {\ensuremath{\kaon^0_{S}}\xspace} 
\def\KL    {\ensuremath{\kaon^0_{L}}\xspace} 
\def\Kstarz  {\ensuremath{\kaon^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{\kaon^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{\kaon^{*+}}\xspace}
\def\Kstarm  {\ensuremath{\kaon^{*-}}\xspace}
\def\Kstarpm {\ensuremath{\kaon^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{\kaon^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}

%% Heavy mesons

\def\D       {\ensuremath{\PD}\xspace}
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em \PD}{}\xspace}% do NOT use ensuremath here
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{\D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{\D^+}\xspace}
\def\Dm      {\ensuremath{\D^-}\xspace}
\def\Dpm     {\ensuremath{\D^\pm}\xspace}
\def\Dmp     {\ensuremath{\D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{\D^*}\xspace}
\def\Dsttt   {\ensuremath{\Dstar(2010)^+}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{\D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{\D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{\D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{\D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{\D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{\D^+_\squark}\xspace}
\def\Dsp     {\ensuremath{\D^+_\squark}\xspace}
\def\Dsm     {\ensuremath{\D^-_\squark}\xspace}
\def\Dspm    {\ensuremath{\D^{\pm}_\squark}\xspace}
\def\Dsmp    {\ensuremath{\D^{\mp}_\squark}\xspace}
\def\Dss     {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssp    {\ensuremath{\D^{*+}_\squark}\xspace}
\def\Dssm    {\ensuremath{\D^{*-}_\squark}\xspace}
\def\Dsspm   {\ensuremath{\D^{*\pm}_\squark}\xspace}
\def\Dssmp   {\ensuremath{\D^{*\mp}_\squark}\xspace}

\def\B       {\ensuremath{\PB}\xspace}
\def\Bbar    {\ensuremath{\kern 0.18em\overline{\kern -0.18em \PB}{}}\xspace}% do NOT use ensuremath here
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BBbar   {\ensuremath{\B\Bbar}\xspace} 
\def\Bz      {\ensuremath{\B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bu      {\ensuremath{\B^+}\xspace}
\def\Bub     {\ensuremath{\B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{\B^\pm}\xspace}
\def\Bmp     {\ensuremath{\B^\mp}\xspace}
\def\Bd      {\ensuremath{\B^0}\xspace}
\def\Bs      {\ensuremath{\B^0_\squark}\xspace}
\def\Bsb     {\ensuremath{\Bbar^0_\squark}\xspace}
\def\Bdb     {\ensuremath{\Bbar^0}\xspace}
\def\Bc      {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcp     {\ensuremath{\B_\cquark^+}\xspace}
\def\Bcm     {\ensuremath{\B_\cquark^-}\xspace}
\def\Bcpm    {\ensuremath{\B_\cquark^\pm}\xspace}

%% Onia

\def\jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\Ppsi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\Ppsi(3770)}\xspace}
\def\etac     {\ensuremath{\Peta_\cquark}\xspace}
\def\chiczero {\ensuremath{\Pchi_{\cquark 0}}\xspace}
\def\chicone  {\ensuremath{\Pchi_{\cquark 1}}\xspace}
\def\chictwo  {\ensuremath{\Pchi_{\cquark 2}}\xspace}
\def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

\def\chic  {\ensuremath{\Pchi_{c}}\xspace}

%% Baryons

\def\proton      {\ensuremath{\Pp}\xspace}
\def\antiproton  {\ensuremath{\overline \proton}\xspace}
\def\neutron     {\ensuremath{\Pn}\xspace}
\def\antineutron {\ensuremath{\overline \neutron}\xspace}

\def\Deltares {\ensuremath{\PDelta}\xspace}
\def\Deltaresbar{\ensuremath{\overline \Deltares}\xspace}
\def\Xires {\ensuremath{\PXi}\xspace}
\def\Xiresbar{\ensuremath{\overline \Xires}\xspace}
\def\L {\ensuremath{\PLambda}\xspace}
\def\Lbar {\ensuremath{\kern 0.1em\overline{\kern -0.1em\PLambda}}\xspace}
\def\Lambdares {\ensuremath{\PLambda}\xspace}
\def\Lambdaresbar{\ensuremath{\Lbar}\xspace}
\def\Sigmares {\ensuremath{\PSigma}\xspace}
\def\Sigmaresbar{\ensuremath{\overline \Sigmares}\xspace}
\def\Omegares {\ensuremath{\POmega}\xspace}
\def\Omegaresbar{\ensuremath{\overline \Omegares}\xspace}

\def\Lz      {\ensuremath{\L^0}\xspace}
\def\Lzbar   {\ensuremath{\Lbar^0}\xspace}
\def\Lc      {\ensuremath{\L^+_\cquark}\xspace}
\def\Lcbar   {\ensuremath{\Lbar^-_\cquark}\xspace}
\def\Lb      {\ensuremath{\L^0_\bquark}\xspace}
\def\Lbbar   {\ensuremath{\Lbar^0_\bquark}\xspace}

%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%

%% Decays
\def\BF         {{\ensuremath{\cal B}\xspace}}
\def\BRvis      {{\ensuremath{\BR_{\rm{vis}}}}}
\def\BR         {\BF}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}

%% EW theory, groups
\def\grpsuthree {\ensuremath{\mathrm{SU}(3)}\xspace}
\def\grpsutw    {\ensuremath{\mathrm{SU}(2)}\xspace}
\def\grpuone    {\ensuremath{\mathrm{U}(1)}\xspace}

\def\ssqtw {\ensuremath{\sin^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\csqtw {\ensuremath{\cos^{2}\!\theta_{\mathrm{W}}}\xspace}
\def\stw   {\ensuremath{\sin\theta_{\mathrm{W}}}\xspace}
\def\ctw   {\ensuremath{\cos\theta_{\mathrm{W}}}\xspace}
\def\ssqtwef {\ensuremath{{\sin}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\csqtwef {\ensuremath{{\cos}^{2}\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\stwef {\ensuremath{\sin\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\ctwef {\ensuremath{\cos\theta_{\mathrm{W}}^{\mathrm{eff}}}\xspace}
\def\gv    {\ensuremath{g_{\mbox{\tiny V}}}\xspace}
\def\ga    {\ensuremath{g_{\mbox{\tiny A}}}\xspace}

\def\order   {\ensuremath{\mathcal{O}}\xspace}
\def\ordalph {\ensuremath{\mathcal{O}(\alpha)}\xspace}
\def\ordalsq {\ensuremath{\mathcal{O}(\alpha^{2})}\xspace}
\def\ordalcb {\ensuremath{\mathcal{O}(\alpha^{3})}\xspace}

%% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}
\def\qsq       {\ensuremath{q^2}\xspace}

%% CKM, CP violation

\def\eps   {\ensuremath{\varepsilon}\xspace}
\def\epsK  {\ensuremath{\varepsilon_K}\xspace}
\def\epsB  {\ensuremath{\varepsilon_B}\xspace}
\def\epsp  {\ensuremath{\varepsilon^\prime_K}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}

\def\Vud  {\ensuremath{V_{\uquark\dquark}}\xspace}
\def\Vcd  {\ensuremath{V_{\cquark\dquark}}\xspace}
\def\Vtd  {\ensuremath{V_{\tquark\dquark}}\xspace}
\def\Vus  {\ensuremath{V_{\uquark\squark}}\xspace}
\def\Vcs  {\ensuremath{V_{\cquark\squark}}\xspace}
\def\Vts  {\ensuremath{V_{\tquark\squark}}\xspace}
\def\Vub  {\ensuremath{V_{\uquark\bquark}}\xspace}
\def\Vcb  {\ensuremath{V_{\cquark\bquark}}\xspace}
\def\Vtb  {\ensuremath{V_{\tquark\bquark}}\xspace}

\def\Vudm  {\ensuremath{|V_{\uquark\dquark}|}\xspace}
\def\Vcdm  {\ensuremath{|V_{\cquark\dquark}|}\xspace}
\def\Vtdm  {\ensuremath{|V_{\tquark\dquark}|}\xspace}
\def\Vusm  {\ensuremath{|V_{\uquark\squark}|}\xspace}
\def\Vcsm  {\ensuremath{|V_{\cquark\squark}|}\xspace}
\def\Vtsm  {\ensuremath{|V_{\tquark\squark}|}\xspace}
\def\Vubm  {\ensuremath{|V_{\uquark\bquark}|}\xspace}
\def\Vcbm  {\ensuremath{|V_{\cquark\bquark}|}\xspace}
\def\Vtbm  {\ensuremath{|V_{\tquark\bquark}|}\xspace}

%% Oscillations

\newcommand{\dm}{\ensuremath{\Delta m}\xspace}
\newcommand{\dms}{\ensuremath{\Delta m_{\squark}}\xspace}
\newcommand{\dmd}{\ensuremath{\Delta m_{\dquark}}\xspace}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}\xspace}
\newcommand{\DGs}{\ensuremath{\Delta\Gamma_{\squark}}\xspace}
\newcommand{\DGd}{\ensuremath{\Delta\Gamma_{\dquark}}\xspace}
\newcommand{\Gs}{\ensuremath{\Gamma_{\squark}}\xspace}
\newcommand{\Gd}{\ensuremath{\Gamma_{\dquark}}\xspace}

\newcommand{\MBq}{\ensuremath{M_{\B_\quark}}\xspace}
\newcommand{\DGq}{\ensuremath{\Delta\Gamma_{\quark}}\xspace}
\newcommand{\Gq}{\ensuremath{\Gamma_{\quark}}\xspace}
\newcommand{\dmq}{\ensuremath{\Delta m_{\quark}}\xspace}
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_{\rm H}}\xspace}

% \newcommand{\ACP}{\ensuremath{{\cal A}^{\CP}}\xspace}
% \newcommand{\SCP}{\ensuremath{{\cal S}^{\CP}}\xspace}
\newcommand{\ACP}{\ensuremath{A}\xspace}
\newcommand{\SCP}{\ensuremath{S}\xspace}
\newcommand{\Adir}{\ensuremath{{\cal A}^{\rm dir}}\xspace}
\newcommand{\Amix}{\ensuremath{{\cal A}^{\rm mix}}\xspace}
\newcommand{\ADelta}{\ensuremath{{\cal A}^\Delta}\xspace}

%% Tagging
\newcommand{\eff}{{\ensuremath{\varepsilon}}\xspace}
\newcommand{\efftag}{{\ensuremath{\varepsilon_{\rm tag}}}\xspace}
\newcommand{\mistag}{\ensuremath{\omega}\xspace}
\newcommand{\effeff}{{\ensuremath{\varepsilon_{\rm eff}}}\xspace}
\newcommand{\efftageff}{{\ensuremath{\varepsilon^{\rm eff}_{\rm tag}}}\xspace}

%% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\rm\,#1}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\rm m}\xspace}
\def\muma {\ensuremath{\,\upmu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mub{\ensuremath{\rm \,\upmu b}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\nb {\ensuremath{\rm \,nb}\xspace}
\def\invnb {\ensuremath{\mbox{\,nb}^{-1}}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\ab   {\ensuremath{\mbox{\,ab}}\xspace}
\def\invab   {\ensuremath{\mbox{\,ab}^{-1}}\xspace}

%% Time 
\def\sec  {\ensuremath{\rm {\,s}}\xspace}
\def\ms   {\ensuremath{{\rm \,ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu{\rm s}}\xspace}
\def\ns   {\ensuremath{{\rm \,ns}}\xspace}
\def\ps   {\ensuremath{{\rm \,ps}}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

\def\mhz  {\ensuremath{{\rm \,MHz}}\xspace}
\def\khz  {\ensuremath{{\rm \,kHz}}\xspace}
\def\hz   {\ensuremath{{\rm \,Hz}}\xspace}

\def\invps{\ensuremath{{\rm \,ps^{-1}}}\xspace}

\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}

%% Temperature
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}

%% Angles
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}
\def\rad{\ensuremath{\rm \,rad}\xspace}

%% Material lengths, radiation
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\def\mip {MIP\xspace}
\def\neutroneq {\ensuremath{\rm \,n_{eq}}\xspace}
\def\neqcmcm {\ensuremath{\rm \,n_{eq} / cm^2}\xspace}
\def\kRad {\ensuremath{\rm \,kRad}\xspace}
\def\MRad {\ensuremath{\rm \,MRad}\xspace}
\def\ci {\ensuremath{\rm \,Ci}\xspace}
\def\mci {\ensuremath{\rm \,mCi}\xspace}

%% Uncertainties
\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}

%% Maths
\def\order{{\ensuremath{\cal O}}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\chisqndf}{\ensuremath{\chisq/\mathrm{ndf}}\xspace}
\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}

\newcommand{\mean}[1]{\ensuremath{\left\langle #1 \right\rangle}} % {x}
\newcommand{\abs}[1]{\ensuremath{\left\|#1\right\|}} % {x}
\newcommand{\Real}{\ensuremath{\mathcal{R}e}\xspace}
\newcommand{\Imag}{\ensuremath{\mathcal{I}m}\xspace}

\def\sPlot{\mbox{\em sPlot}~}
\def\sWeight{\mbox{\em sWeight}~}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Energy, Momenta
\def\Ebeam {\ensuremath{E_{\mbox{\tiny BEAM}}}\xspace}
\def\sqs   {\ensuremath{\protect\sqrt{s}}\xspace}

\def\pt         {\mbox{$p_{\rm T}$}\xspace}
\def\et         {\mbox{$E_{\rm T}$}\xspace}

\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\evtgen   {\mbox{\textsc{EvtGen}}\xspace}
\def\pythia    {\mbox{\textsc{Pythia8}}\xspace}
\def\kkmc     {\mbox{\textsc{KKMC}}\xspace}
\def\geant     {\mbox{\textsc{Geant4}}\xspace}
\def\photos   {\mbox{\textsc{Photos}}\xspace}
\def\tauola    {\mbox{\textsc{TAUOLA}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\pyroot   {\mbox{\textsc{PyRoot}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}}\xspace}
\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{Fortran}}\xspace}

%%%%%%%%%%%%%%%
% Special Text 
%%%%%%%%%%%%%%%
\newcommand{\eg}{\mbox{\itshape e.g.}\xspace}
\newcommand{\ie}{\mbox{\itshape i.e.}}
\newcommand{\etal}{{\slshape et al.}\xspace}
\newcommand{\etc}{\mbox{\itshape etc.}\xspace}
\newcommand{\cf}{\mbox{\itshape cf.}\xspace}
\newcommand{\ffp}{\mbox{\itshape ff.}\xspace}
\newcommand{\vs}{\mbox{\itshape vs.}\xspace}

%%%%%%%%%%%%%%%%%%%%
% Analysis Specific
%%%%%%%%%%%%%%%%%%%%

% bookkepping
\def\needref{{\color{red}{[Ref needed]}}\xspace}

% luminosity
\def\nbb{\ensuremath{(387\pm 6)\times 10^6}\xspace} % updated 22/02/2023 [coll-members:8741]
\def\lumi{\ensuremath{362\pm2~\invfb}\xspace} % update with final number

% accelerator
\def\betagamma{\ensuremath{\beta\gamma}\xspace}
\def\boost{\ensuremath{0.28}\xspace}

% tagging
\def\bsig{\ensuremath{\B_{\CP}}\xspace}
\def\btag{\ensuremath{\B_{\text{tag}}}\xspace}
\def\qtag{\ensuremath{q} \xspace}
\def\dwtag{\ensuremath{\Delta w} \xspace}
\def\wtag{\ensuremath{w} \xspace}
% \def\mutag{\ensuremath{\mu} \xspace}
\def\mutag{\ensuremath{a^{\rm tag}_{\epsilon}} \xspace}
\def\qf{\ensuremath{q_f}\xspace}

% resolution
\def\dterr{\ensuremath{\sigma_{\dt}} \xspace}
\def\dtres{\ensuremath{\mathcal{R}(\dt-\dtp| \dterr)} \xspace}
\def\dtp{\ensuremath{\dt'}\xspace}

% decay time
\def\tcp{\ensuremath{t_{\CP}}\xspace}
\def\ttag{\ensuremath{t_{\text{tag}}}\xspace}
\def\fcp{\ensuremath{f_{\CP}}\xspace}
\def\ftag{\ensuremath{f_{\text{tag}}}\xspace}
\def\lcp{\ensuremath{\ell_{\CP}}\xspace}
\def\ltag{\ensuremath{\ell_{\text{tag}}}\xspace}

% decay channels
\def\jpsiks{\ensuremath{\Bz \ra \jpsi \KS}\xspace}
\def\jpsikz{\ensuremath{\Bz \ra \jpsi \Kz}\xspace}
\def\phiks{\ensuremath{\Bz \ra \phi \KS}\xspace}
\def\phikz{\ensuremath{\Bz \ra \phi \Kz}\xspace}
\def\phikp{\ensuremath{\Bp \ra \phi \Kp}\xspace}
\def\phikstar{\ensuremath{\Bz \ra \phi \Kstarz}\xspace}
\def\nonres{\ensuremath{\Bz \ra \Kp \Km \KS}\xspace}
\def\kspipi{\ensuremath{\KS \to \pip \pim}\xspace}
\def\phikk{\ensuremath{\phi \to \Kp \Km}\xspace}
\def\dpi{\ensuremath{\Bz \ra  D^{(*)-}\pip}\xspace}
\def\dzpip{\ensuremath{\Bp \ra  \Dzb\pip}\xspace}
\def\kspiz{\ensuremath{\Bz \ra \KS \piz}\xspace}
\def\ksksks{\ensuremath{\Bz \ra \KS \KS \KS}\xspace}
\def\kskskp{\ensuremath{\Bp \ra \KS \KS \Kp}\xspace}

% quark transitions
\def\ccs{\ensuremath{\bquark \to \cquark \cquarkbar \squark}\xspace}
\def\qqs{\ensuremath{\bquark \to \qqbar \squark}\xspace}
\def\sss{\ensuremath{\bquark \to \squark \squarkbar \squark}\xspace}

% CKM parameters
\def\phione{\ensuremath{\phi_1}\xspace}
\def\Vij {\ensuremath{V_{ij}}\xspace}

% Mixing parameters
\def\dt{\ensuremath{\Delta t}\xspace}
\def\taud{\ensuremath{\tau_{\Bz}}\xspace}
\def\etaf{\ensuremath{\eta_f}\xspace}
\def\sintpo{\ensuremath{\sin 2\phione}\xspace}

\def\Phi{\ensuremath{\phi}\xspace}

% invariant masses
\def\mkk{\ensuremath{m (\Kp\Km)}\xspace}
\def\mpipi{\ensuremath{m (\pip\pim)}\xspace}
\def\mbc{\ensuremath{M_{\text{bc}}}\xspace}
\def\deltae{\ensuremath{\Delta E}\xspace}
\def\cosh{\ensuremath{\cos \theta_{H}}\xspace}
\def\ocs{\ensuremath{\mathcal{O}^{'}_{CS}}\xspace}
\def\obdt{\ensuremath{\mathcal{O}_{CS}}\xspace}
\def\ebeam{\ensuremath{E_{\text{beam}}^{*}}\xspace}
\def\pstar{\ensuremath{p_B^*}\xspace}
\def\estar{\ensuremath{E_B^*}\xspace}

% vertex fit
\def\treefit   {\ensuremath{\texttt{TreeFitter}}\xspace}
\def\rave   {\ensuremath{\texttt{Rave}}\xspace}

% cp par
\def\acpnrk{\ensuremath{A_{CP}^{K^+K^- \KS}}\xspace}
\def\scpnrk{\ensuremath{S_{CP}^{K^+K^- \KS}}\xspace}

% yields
\newcommand{\notepath}{/Users/michele/Work/gitlab/b2phiks-note/belle2note}
\def\nqqb{\ensuremath{\input{results/cpfit/nqqb_phiks.tex}}\xspace}
\def\nphik{\ensuremath{\input{results/cpfit/nphik_phiks.tex}}\xspace}
\def\nkskk{\ensuremath{\input{results/cpfit/nr_phiks.tex}}\xspace}
\def\acpphiks{\ensuremath{\input{results/cpfit/acp_phiks.tex}}\xspace}
\def\scpphiks{\ensuremath{\input{results/cpfit/scp_phiks.tex}}\xspace}
\def\acpphikssyst{\ensuremath{\input{results/cpfit/acp_phiks_syst.tex}}\xspace}
\def\scpphikssyst{\ensuremath{\input{results/cpfit/scp_phiks_syst.tex}}\xspace}
\def\phikscorr{\ensuremath{\input{results/cpfit/corr_acp_scp_phiks.tex}}\xspace}

\def\nqqbp{\ensuremath{\input{results/cpfit/nqqb_phikp.tex}}\xspace}
\def\nphikp{\ensuremath{\input{results/cpfit/nphik_phikp.tex}}\xspace}
\def\nkskkp{\ensuremath{\input{results/cpfit/nr_phikp.tex}}\xspace}
\def\acpphikp{\ensuremath{\input{results/cpfit/acp_phikp.tex}}\xspace}
\def\scpphikp{\ensuremath{\input{results/cpfit/scp_phikp.tex}}\xspace}
\def\phikpcorr{\ensuremath{\input{results/cpfit/corr_acp_scp_phikp.tex}}\xspace}

% BDT
\def\xgboost{\ensuremath{\texttt{XGBoost}}\xspace}

